The ViP2P Platform: XML Views in P2P

The growing volumes of XML data sources on the Web or produced by enterprises, organizations etc. raise many performance challenges for data management applications. In this work, we are concerned with the distributed, peer-to-peer management of large corpora of XML documents, based on distributed hash table (or DHT, in short) overlay networks. We present ViP2P (standing for Views in Peer-to-Peer), a distributed platform for sharing XML documents based on a structured P2P network infrastructure (DHT). At the core of ViP2P stand distributed materialized XML views, defined by arbitrary XML queries, filled in with data published anywhere in the network, and exploited to efficiently answer queries issued by any network peer. ViP2P allows user queries to be evaluated over XML documents published by peers in two modes. First, a long-running subscription mode, when a query can be registered in the system and receive answers incrementally when and if published data matches the query. Second, queries can also be asked in an ad-hoc, snapshot mode, where results are required immediately and must be computed based on the results of other long-running, subscription queries. ViP2P innovates over other similar DHT-based XML sharing platforms by using a very expressive structured XML query language. This expressivity leads to a very flexible distribution of XML content in the ViP2P network, and to efficient snapshot query execution. ViP2P has been tested in real deployments of hundreds of computers. We present the platform architecture, its internal algorithms, and demonstrate its efficiency and scalability through a set of experiments. Our experimental results outgrow by orders of magnitude similar competitor systems in terms of data volumes, network size and data dissemination throughput.

==> figures/experiments/data/data_transfer_pipe <==
set size ratio 0 1,1 
set size ratio 0 0.7,0.7
set ylabel "Time (ms)"
#set timestamp top
set datafile separator "," 
set xlabel "Size of document (MB)"
set ylabel "Time (sec)"
set key top left
set size 0.5,0.5
set xrange [100:500] 

set grid y


set xtics 100

set terminal postscript eps enhanced 

set xrange [50:550] 
set boxwidth 20


set output "../data_transfer_pipe.eps"


plot  	"data_transfer_pipe.csv" using ($1-25):($4/1000) title "Data exchange time" with boxes fs pattern 1, \
	"data_transfer_pipe.csv" using 1:($2/1000) title "BDB storage time" with boxes fs pattern 2, \
	"data_transfer_pipe.csv" using ($1+25):($3/1000) title "Extraction time" with boxes fs solid
	



==> figures/experiments/data/many_publishers_one_consumer_vary_data <==
set size ratio 0 0.6,0.6
set datafile separator ","
set xtics (64,512,1024,2048,3200)
set xlabel "Size of data published (MB)"
set key top left
set terminal postscript eps enhanced 
set size 0.605,0.505
set grid y

set ylabel "View materialization time (sec)"

set output "../many_publishers_one_consumer_vary_data.eps"

plot "many_publishers_one_consumer_vary_data.csv" using 1:($2/1000) title "Sequential tuple receiving" with lp lt 1 pt 7, \
"many_publishers_one_consumer_vary_data.csv" using 1:($3/1000) title "Parallel tuple receiving" with lp lt 1 pt 2







==> figures/experiments/data/parallel_vs_sequential_extraction <==
set size ratio 0 1,1 
set size ratio 0 0.75,0.75
set datafile separator "," 
set ylabel "Extraction time (sec)"
set xlabel "Number of patterns"
set grid y

set style data histogram
set style histogram cluster gap 1
set style fill solid border -1
set boxwidth 0.6
set key top left
set size 0.5,0.5

set yrange [0:50]

set terminal postscript eps enhanced 
set output "../parallel_vs_sequential_extraction.eps"


plot  	"parallel_vs_sequential_extraction.csv" using ($2/1000):xtic(1) ti col fs pattern 5,\
  	"parallel_vs_sequential_extraction.csv" using ($3/1000):xtic(1) ti col


==> figures/experiments/data/query_response_views_vs_documents <==
set size ratio 0 1,1 
set size ratio 0 0.6,0.6
set datafile separator "," 
set ylabel "Query response time (ms)"
set xlabel "Number of data sources"
set key below
set grid y

set terminal postscript eps enhanced 
set output "../query_response_views_vs_documents.eps"

plot  	"query_response_views_vs_documents.csv" using 1:2 title "Documents" with lp  lt 1 pt 7, \
	"query_response_views_vs_documents.csv" using 1:3 title "Views" with lp  lt 1 pt 8




==> figures/experiments/data/views_per_peer <==
set size ratio 0 1,1 
set size ratio 0 0.6,0.6
set datafile separator ","
set xtics 4
#set timestamp top
set xlabel "Number of views that a publisher contributes to"

set key at 46,185
set size 0.72,0.51




set terminal postscript eps enhanced 

set ylabel "Time (sec)"
set output "../views_per_peer.eps"
plot "views_per_peer.csv" using 1:($2/1000) title "Mat. time: sequential tuple sending" with lp, \
"views_per_peer.csv" using 1:($4/1000) title "Mat. time: parallel tuple sending" with lp, \
"views_per_peer.csv" using 1:($3/1000) title "Tuple extraction time" with lp







==> removed_experiments.tex <==
\subsubsection{Materialization of documents contributing to one view}
\AK{clean this mess}
In this we analyzed the variation of view materialization time while varying number of documents for a view. This experiment is different from the previous experiment because here we have more than one view in the network. The XML file used for this experiment is depicted in the figure~\ref{file3}. View used for the experiment is $//size//[REPLACEME_{cont},people_{cont}]$ and it will the extract the whole document. If $n$ documents attack a peer then REPLACEME for document and view will be peerID$/n$ and view is saved with node where peerID$\%n=0$.  
\begin{figure}[ht!]
  \begin{center}
	\begin{tikzpicture}[level distance=10mm]
	\tikzstyle{edge from parent}=[draw]
		\hspace{-20mm}
	\node {$site$}
		child {
			node {$replaceme$}
			child { 
				node {$data$}
				edge from parent node[left] {\tiny{\emph{1000}}}
			}
			edge from parent node[left] {\tiny{\emph{100}}}
		}
		child { 	
			node { $people$ }
			child { 
				node {$data$}
				edge from parent node[right] {\tiny{\emph{1000}}}
			}
			edge from parent node[right] {\tiny{\emph{100}}}
		};
		\hspace{40mm}
		\tikzstyle{edge from parent}=[thick,draw,double]
		\node {$site$}
			child { node {$~~~replaceme_{cont}~~~~~$} }
			child { node {$~~~~~~people_{cont}$} };
	\end{tikzpicture}
	\vspace{-2mm}
	\caption{\small Structure of XML document (left); View used (right).}
  \label{file3}
  \end{center}
\end{figure}

The specifications for the experiment are given in the table below. 250 nodes located at lille, sophia and lyon are used for the experiment and number of peers per physical machines are 1. Total size of data in the network is 500 Mb and 2 Mb of data is present with each peer. Number of documents attacking a view is varied from 12 to 120 with increment of 12.

\noindent The parameters characterizing this experiment are given in the table below:
\begin{center}
  \begin{tabular}[h!]{ c p{2mm} c  p{2mm} c p{2mm} c p{2mm} c p{2mm} c p{3mm} c p{3mm} c p{3mm} }
    $|P|$ & & $|{\phi}|$ & & $|P_{D}|$ & &  $|V|$& &  $|P_{V}|$& & $|D|$ & &  $|D_v|$& &  $|d|$ \\\hline
	240 & &  240 & &  240 & & \{20,10,5,4,2\}  & &  1 & &  240 & &  \{12,24,48,60,120\} & &  1 \\
	\end{tabular}
\end{center}

It is clear from Figure~\ref{attkpeers} that as numbers of documents attacking a view increases view materialization time increases. We have also analysed the performance from another perspective. As we are having many views in this experiment and  documents correspond to a single view only therefore there are many subnetworks formed in the network. All the subnetworks formed are completely disjoint. More number of subnetworks means more parallel processing and therefore time need for view materialization decreases as we increase more number of networks. One major reason for decreasing the time is that when there are large subnetworks then data associated with view materialization is also small. The variation of view materialization for this is given in figure~\ref{subnetworks} 

\begin{figure*}[ht!]
	\includegraphics[width=0.5\textwidth]{figures/experiments/peers_per_view}
	\includegraphics[width=0.5\textwidth]{figures/experiments/subnetworks}

  	\caption{\small View materialization time according to the number of peers contributing to a view (left);
 View materialization time with variation of number of subnetworks (right)
}
	\label{attkpeers}
\end{figure*}

\subsubsection{Publishing of documents by varying number of publishers}
In this experiment, we study the materialization time when the network has to absorb 250MBs of documents of small size. The number of peers that publish data (\emph{document publishers} or \emph{publishers}) varies. Only one view is present in the network and all document publishers contribute data to it.

\noindent The parameters of this experiment are summarized in the table below:
\begin{center}
  \begin{tabular}[h!]{ c p{5mm} c  p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} }
    $|P|$ & & $|{\phi}|$ & & $|P_{D}|$ & & $|V|$ & & $|P_{V}|$ & & $|D|$ & & $|D_{v}|$ & & $|d|$ \\\hline
	500 & & 250 & & \{50,100,$\ldots$,500\} & & 1 & & 1 & & 126K & & 126K & & ~20KB \\
  \end{tabular}
\end{center}


\noindent Figure \ref{fixed_docs_varying_peers_holding_them} depicts the results. The materialization time when the documents are published by 50 peers is about 168 seconds. As the number of publishers increases, the materialization time falls to 148 seconds (when the publishers are 200). This is expected, since the more publishers publish documents, the more they share the effort of extracting data from the documents. On the other hand when the publishers increase to 250, we also notice an increase to the materialization time. This is due to the fact that the publishers are reaching the point that  they cause overload to the view holder.

\begin{figure}[ht!]
  \begin{center}
    \includegraphics{figures/experiments/fixed_docs_varying_peers_holding_them}
  \end{center}
  \caption{\small View materialization while varying number of peers holding 250 MB of data}
  \label{fixed_docs_varying_peers_holding_them}
\end{figure}

Notice that starting from 300 publishers and upwards, the materialization time increases dramatically. This is due to the fact that two peers share the same physical machine and the resources of the physical machine are limited. Thus, the machine starts to swap out memory pages leading to big increase of the time needed to extract data from the document. We have left this figure as is in purpose: to show that running more than 2 peers on a physical machine leads to unexpected results. From now on, all experiments are going to include only one peer per physical machine.


\subsubsection{Data extraction and local storage time}
In this experiment we study the time it takes to ($i$)~apply a pattern on a document to extract the corresponding tuples, ($ii$)~send those tuples to the view holder and ($iii$)~store  the set of tuples in the view holder's BerkeleyDB-based store. 

\noindent The following parameters are used:
\begin{center}
  \begin{tabular}[h!]{ c p{5mm} c  p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} }
    % \hline
    ~$|P|$ ~& & ~$|{\phi}|$ ~& & $|P_{D}|$& &$|V|$& &$|P_{V}|$& &$|D|$& &$|D_{V}|$& &$|d|$\\ \hline
	2 & & 2 & & 1 & & \{1,2\} & & 1 & & 1 & & 1 & & \{0.03 \ldots 3.7MB\} \\ %\hline
  \end{tabular}
\end{center}

We use two views $v_1$, $v_2$. $v_1$ is a low selectivity view, whose number of tuples extracted, increase linearly with respect to the size of the document. $v_2$ is a high-selectivity view which extracts only one tuple from the document. The shapes of the views $v_1$, $v_2$ and the document used, are depicted in Figure ~\ref{selectivity-views}.

\begin{figure}[h!]
\begin{center}
	\begin{tikzpicture}[level distance=10mm]
	\tikzstyle{edge from parent}=[thick,double,draw]
	
	\hspace{-30mm}
	
	\node {$a_{id}$}
		child {node {$b_{@id="1"}$}};
	
	\hspace{30mm}
	
	\node {$a_{id}$}
		child {node {$b_{id}$}};	
	
	\hspace{30mm}
	
	\tikzstyle{edge from parent}=[draw]
	\node {$a$}
		child {
			node {$b$}
			edge from parent node[right] {\tiny{\emph{200.000}}}
		};	
		
	\end{tikzpicture}
	\vspace{-3mm}
	\caption{\small High selectivity view $v_1$ (left); Low selectivity view $v_2$ (center); Summary of the document from which data were extracted (right).}
  \label{selectivity-views}
\end{center}
\end{figure}

We study the time taken by these operations as a function of the input document size. Figure \ref{materialization-high-low} depicts the individual times needed for the materialization of the two views to be performed. 


\begin{figure*}[ht!]
\includegraphics[width=0.5\textwidth]{figures/experiments/materialization_high_selectivity}
 \includegraphics[width=0.5\textwidth]{figures/experiments/materialization_low_selectivity}
  \caption{\small Materialization of high selectivity view $v_2$ (left); Materialization of low selectivity view $v_1$ (right).}
  \label{materialization-high-low}
\end{figure*}

We observe that extraction time is linear to the size of the document which is coherent with the stack based algorithm~\cite{DBLP:conf/SIGMOD/BrunoKS02} used for the extraction. BerkeleyDB storage time is proportional with the extracted data size and comparable to the extraction time for the low selectivity view. In this experiment, the network connecting the two peers was a 1GBit LAN. Since the data exchange time is very low, we conclude that the extraction time and the BerkeleyDB storage time are the two bottlenecks in the materialization process.






\newpage
\subsection{Optionally presented experiments}
\subsubsection{Materialization of documents with varying size of the DHT network}
In this experiment we study the DHT network's size impact to the materialization process. The size of the DHT network varies keeping the number of peers holding data (and the data themselves) constant. To change the size of DHT extra -idle- nodes are added in the network.

\noindent The parameters characterizing this experiment are given in the table below:
\begin{center}
  \begin{tabular}[h!]{ c p{2mm} c  p{2mm} c p{2mm} c p{2mm} c p{2mm} c p{3mm} c p{3mm} c p{3mm} }
    $|P|$ & & $|{\phi}|$& & $|P_{D}|$& & $|V|$& & $|P_{V}|$& & $|D|$& & $|D_{v}|$& & $|d|$ \\ \hline
\{50,\ldots,250\} & & \{50,\ldots,250\} & & 50 & & 1 & & 1 & & \{50,100\} & & \{50,100\} & & 5MB \\
  \end{tabular}
\end{center}

Figure \ref{variable_dht} depicts the experimental results. We observe that the materialization time is not seriously affected by the size of the DHT network. The difference in time noticed (about 13-15 seconds in both 500MBs and 250MBs) is due to the overhead of bootstrapping the network and not due to the increase of the DHT network size.

\begin{figure}[h!]
  \begin{center}
    \includegraphics{figures/experiments/variable_dht}
  \end{center}
\vspace{-4mm}
  \caption{View materialization time when varying the DHT size.}
  \label{variable_dht}
\end{figure}

\subsubsection{Impact of network capacity to materialization time}
In this experiment we study the impact of the network capacity to the materialization process. 250 peers are deployed with one document and one view each. Each of the views matches only one document and each document contributes data to only one view. To study the impact of network capacity we have tested view materialization in two variations:
\begin{itemize}
 \item \textbf{Views and documents located on different peers:} In this variation, the view and its matching document are located on different peers
\item \textbf{Views and documents located in the same peer:} In this variation both the view and its matching document are located on the same peer.
\end{itemize}

\noindent The parameters characterizing this experiment are given below:
\begin{center}
  \begin{tabular}[h!]{ c p{5mm} c  p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} c p{5mm} }
    $|P|$ & & $|{\phi}|$ & & $|P_{D}|$& & $|V|$& &$|P_{V}|$ & &$|D|$ & &$|D_v|$ & &$|d|$ \\\hline
	250 & & 250 & & 250 & & 250 & & 250 & & 250 & & 250 & & \{5,10,20\}MB \\
  \end{tabular}
\end{center}

In both variations, we test view materialization for 1.25, 2.5 and 10GBs of total documents size. In Figure~\ref{materialization_local_vs_remote} we observe that the difference between exchanging the contents of the view does not impact a lot the materialization time (about 10\% impact). This is due to the fact that the nodes in the Grid5000 infrastructure are interconnected with high speed networks and exchanging of data is very fast.

\begin{figure}
  \begin{center}
    \includegraphics[width=3.4in]{figures/experiments/materialization_local_vs_remote}
  \end{center}
  \caption{Comparison of view materialization time between when view is saved remotely and on the same peer.}
  \label{materialization_local_vs_remote}
\end{figure}



























==> rewr-fig-queryplan.tex <==
\begin{tabular}{||c|c||}
\hline\hline

\begin{tabular}{c}
\begin{tabular}{c|c}

% ~&~\\[3mm]

\begin{tabular}{cc}
%----- q1 -----
\raisebox{20mm}{
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\node[pname] {$q_1$}
	child {
		node{$paper$} edge from parent [transparent edge]
		child {
			node[plain]{$author$} edge from parent [descendant]
			child {
				node[plain]{$country_{val}$}
			}
		}
	};
\end{tikzpicture}
}
&
%----- p1 -----
\raisebox{30mm}{
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\node[pname] {$p_1$}
	child {
		node{$nav$} edge from parent [transparent edge]
		child {
			node[plain]{$v_1$} edge from parent [child]
			edge from parent node[above right] {{\tiny$/country_{val}$}}
		}
	};
\end{tikzpicture}
}
\end{tabular}

&

\begin{tabular}{cc}
%----- q2 -----
\raisebox{30mm}{
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\node[pname] {$q_2$}
	child {
		node{$paper$} edge from parent [transparent edge]
		child {
			node[plain]{$author_{val}$} edge from parent [descendant]
		}
		child {
			node[plain]{$year_{val}$}
		}
	};
\end{tikzpicture}
}
&
%----- p2 -----
\begin{tikzpicture}[level/.style={level distance=8mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\raisebox{8.5mm}{
\node[pname] {$p_2$}
	child {
		node{$\sigma_{year \prec paper}$} edge from parent [transparent edge]
		child {
			node[plain]{$\times$}
			child {
				node[plain]{$\sigma_{author \precc paper}$}
				child {
					node[plain]{$\times$}
					child {node[plain]{$v_2$}}
					child {node[plain]{$v_3$}}
				}
			}
			child {node[plain]{$v_4$}}
		}
	};
}
\end{tikzpicture}
\end{tabular}
\vspace{-5mm}
\end{tabular}

\\
\hline

\begin{tabular}{cc}
%----- q4 -----
% \raisebox{8mm}{
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\tikzstyle{level 1}=[sibling distance=2.2cm,level distance=6mm]
\tikzstyle{level 2}=[sibling distance=1.5cm]
\raisebox{-1.5mm}{
\node[pname] {$q_4$}
	child {
		node{$conf$} edge from parent [transparent edge]
		child {
			node[plain]{$paper$}
			child {
				node[plain]{$affiliation_{val}$} edge from parent [descendant]
			}
			child {
				node[plain](year1q){$year$}
			}
		}
	}
	child {
		node{$book$} edge from parent [transparent edge]
		child {
			node[plain](year2q){$year$}
		}
		child {
			node[plain](author1q){$author$}
		}
	}
	child {
		node{$journal$} edge from parent [transparent edge]
		child {
			node[plain]{$tldks$}
			child {
				node[plain](author2q){$author$}
			}
			child {
				node{$title_{val}$}
			}
		}
	};
\draw(year1q) edge[value join] (year2q);
\draw(author1q) edge[value join] (author2q);
}

\end{tikzpicture}
% }
&
%----- p4 -----
\raisebox{1.5mm}{
\begin{tikzpicture}[level/.style={level distance=8mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\node[pname] {$p_4$}
	child {
		node[plain]{$\sigma_{author.val=author.val}$} edge from parent [transparent edge]
		child {
			node[plain]{$\times$} edge from parent [child]
			child {
				node[plain]{$v_5$} edge from parent [child]
			}
			child {
				node[plain]{$v_6$}
			}
		}
	};
\end{tikzpicture}
% \hspace{-2mm}
}
\end{tabular}

\end{tabular}

&

\begin{tabular}{c}
%----- q3 -----
\raisebox{10mm}{
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\raisebox{-1mm}{
\node[pname] {$q_3$}
	child {
		node{$paper$} edge from parent [transparent edge]
		child {
			node[plain]{$author$}
			child {
				node[plain]{$email_{val}$} edge from parent [descendant]
			}
		}
		child {
			node[plain]{$year_{[='2006']}$}
		}
	};
}
\end{tikzpicture}
}

\vspace{-8mm}
\\

%----- p3 -----
~~
\raisebox{0mm}{
\begin{tikzpicture}[level/.style={level distance=8mm},level 1/.style={level distance=7mm},level 2/.style={level distance=10mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\tikzstyle{level 4}=[sibling distance=1.8cm]
\raisebox{2mm}{
\node[pname] {$p_3$}
	child {
		node{\begin{tabular}{c}
			$\sigma_{year \prec paper \wedge}$\\
			$\;\; _{year.val=2006}$
		\end{tabular}} edge from parent [transparent edge]
		child {
			node[plain]{$\times$}
			child {
				node[plain]{$\sigma_{author \precc paper}$}
				child {
					node[plain]{$\times$}
					child {
						node[plain]{$nav$}
						child{
							node[plain]{$v_1$}
							edge from parent node[above right] {{\tiny$~//email_{val}$}}
						}
					}
					child {node[plain]{$v_3$}}
				}
			}
			child {node[plain]{$v_4$}}
		}
	};}
\end{tikzpicture}
}
\end{tabular}

\\
\hline\hline
\end{tabular}


==> rewr-fig-view.tex <==
\begin{tabular}{||c||}
\hline\hline

%----- first line -----
\begin{tabular}{c|c|c|c}

%----- v1 -----
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\raisebox{-4mm}{
\node[pname] {$v_1$}
	child {
		node{$paper_{ID}$} edge from parent [transparent edge]
		child {
			node[plain]{$author_{cont}$} edge from parent [descendant]
		}
	};
}
\end{tikzpicture}

&

%----- v2, v3, v4 -----
\raisebox{5mm}{
\begin{tabular}{c}
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\node[pname] {$v_2$}
	child {
		node{$paper_{ID}$} edge from parent [transparent edge]
	};
\end{tikzpicture}
\\
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\node[pname] {$v_3$}
	child {
		node{$author_{ID,val}$} edge from parent [transparent edge]
	};
\end{tikzpicture}
\\
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\node[pname] {$v_4$}
	child {
		node{$year_{ID,val}$} edge from parent [transparent edge]
	};
\end{tikzpicture}
\end{tabular}
}
&

%----- v4, v5 -----
\raisebox{-2mm}{
\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\tikzstyle{level 1}=[sibling distance=2.2cm,level distance=6mm]
\tikzstyle{level 2}=[sibling distance=1.5cm]
\node[pname] {$v_5$}
	child {
		node{$conf$} edge from parent [transparent edge]
		child {
			node[plain]{$paper$}
			child {
				node[plain]{$affiliation_{val}$} edge from parent [descendant]
			}
			child {
				node[plain](year1v){$year$}
			}
		}
	}
	child {
		node{$book$} edge from parent [transparent edge]
		child {
			node[plain](year2v){$year$}
		}
		child {
			node[plain]{$author_{val}$}
		}
	};

\draw(year1v) edge[value join] (year2v);
\end{tikzpicture}
}

&

\begin{tikzpicture}[level/.style={level distance=10mm},level 1/.style={level distance=7mm}]
\tikzstyle{edge from parent}=[opacity=1,thick,draw]
\raisebox{-2mm}{
\node[pname] {$v_6$}
	child {
		node{$journal$} edge from parent [transparent edge]
		child {
			node[plain]{$tldks$}
			child {
				node[plain]{$author_{val}$}
			}
			child {
				node{$title_{val}$}
			}
		}
	};
}
\end{tikzpicture}

\end{tabular}

\\
\hline\hline
\end{tabular}


==> rewriting.tex <==
\Section{ViP2P query rewriting}
\label{sec:rew-outline}

Once a query is issued to a peer, as described in Section~\ref{sec:platformOverview}, a DHT lookup retrieves the definitions of the existing ViP2P network views which could be used to answer the query. Then, the query peer runs its own algorithm for rewriting the query using the respective materialized views.  The algorithm is presented in~\cite{rewritingICDE2011} and its details are out of the scope of this paper, where we are mainly concerned with the platform and its scalability. To make this paper self-contained, however, we now present %, first, a quick overview of the related works in this area (Section~\ref{sec:related-xml-rew}), and then 
ViP2P rewriting through examples.% in  Section~\ref{sec:rew-examples}.



%---------------------------
\begin{figure}[t!]
\begin{center}
\scalebox{0.75}{
	% \hspace{-12mm}
	\input{rewr-fig-view}
}
\caption{View Pool}
\end{center}
\label{fig:rewr-views}
\end{figure}
%---------------------------


Our rewriting algorithm identifies equivalent rewritings for tree pattern queries (corresponding to an XQuery dialect), using multiple views expressed in the same language. Unlike~\cite{Onose06,Tatarinov}, it uses node identifiers to join multiple views. It differs from~\cite{DBLP:conf/vldb/ArionBMP07} in that it does not require any knowledge about the structure of the XML database, and can be seen as extending~\cite{Cautis08,DBLP:conf/icde/TangYOCW08} to a more expressive view and query language. Moreover, by design, our algorithm only finds {\em minimal rewritings}, i.e., those from which no view can be removed while still preserving the equivalence between the rewriting and the initial query. Rewriting minimality is a desirable feature from a performance perspective, and in particular in our distributed setting where shipping data from remote views may be expensive.

Our overall approach is to build rewritings under the form of logical algebraic plans, which are translated into physical plans through a dedicated cost-based optimization step. This allows ViP2P to take advantage of many efficient optimization and execution techniques in distributed- and XML-databases. 


%---------------------------
\begin{figure}[t!]
\begin{center}
\scalebox{0.63}{
	\input{rewr-fig-queryplan}
}
\caption{Sample queries and rewritings.}
\end{center}
\label{fig:rewr-queriesplans}
\end{figure}
%---------------------------


\vspace{1mm}
\noindent \textbf{XPath navigation}
We consider a set of queries shown in Figure~\ref{fig:rewr-queriesplans} and the views from Figure~\ref{fig:rewr-views}. Query $q_1$ asks for the countries of the authors of all papers. Although $v_1$ does not explicitly store this information, it does store the whole content (subtree) of the authors of the papers. Thus, as depicted by the rewriting plan $p_1$ of Figure~\ref{fig:rewr-queriesplans}, we can apply the $nav$ operator, which performs a navigation inside the XML author subtree stored by $v_1$, searching for children labeled country, and answer $q_1$.

\vspace{1mm}
\noindent \textbf{Joining views}
The second query $q_2$ demands the text values ($val$) of the papers' authors and publication years. Assume that the views $v_2$, $v_3$ and $v_4$ are available to rewrite this query. Each of them stores the structural IDs~\cite{DBLP:conf/icde/Al-KhalifaJPWKS02} of the three nodes that participate in $q_2$. To this end, we can combine the three views through structural joins to retrieve the rewriting expression $p_2$. In particular, $v_2$ is first joined with $v_3$ ensuring that the paper is an ancestor of the author and then the resulting expression is joined with $v_4$ under the condition that the paper is the parent of the year. In $p_2$, a structural join between two views is depicted as a selection ($\sigma_{pred}$) over the cartesian product ($\times$) of the two views. The $pred$icate of the selection enforces this relationship between the nodes, based on their structural ({\em start, end, depth}) IDs, as explained in Section~\ref{sec:views-queries}. The $\prec$ is the parent comparison operator, returning true if the right-hand argument is the father of left-hand one. Likewise, $\precc$ denotes the ancestor comparison operator.

\vspace{1mm}
\noindent \textbf{A more complex case}
Query $q_3$ seeks the e-mails of the authors of the papers published in 2006. The rewriting expression $p_3$ first navigates in $v_1$ to find the e-mails of the authors and then joins the intermediate result with $v_3$ to get the year of the papers and filter out those that were not published in 2006.

\vspace{1mm}
\noindent \textbf{Value joins}
The joined tree pattern query $q_4$ asks for the affiliation of the conference papers published the same year with a book that has the same author with a TLDKS paper, as well as the title of these books.
To rewrite $q_4$, we combine the joined tree pattern view $v_5$ with the single tree pattern view $v_6$ through a value join, imposing that the two views have the same $val$ for their author nodes, through the selection appearing at the top of $p_3$.

Notice that through the value joins, one can ask for (and respectively store, in the case of the views) data that derive from different documents and lead to significant flexibility.


%\vspace{1mm}
%\noindent \textbf{Fall-back option: coarse granularity views} Our main focus in ViP2P is on materializing rich, fine-granularity views in the hope that views stored by some peers can be used to compute the results of queries potentially of other peers. The materialization, indexing and lookup of such views has been discussed in the previous Sections.

%In some cases, however, appropriate views may not be available for a given query. As a fall-back solution only, ViP2P also supports {\em one-node views at document granularity}. Thus, for each element name or keyword appearing in some XML document, a peer is randomly designated to store the URIs of all published documents which contain an occurrence of the respective name or keyword. An example is provided by the views $v_5,v_6,v_7$ in Figure~\ref{fig:rewr-views} which can also be used to answer $q_2$. One can intersect the views to learn the URIs of all documents simultaneously containing the three element names, and then ship $q_2$ to all the peers holding these documents and ask them to evaluate the query.

%One-node document-granularity views can be seen as  a  simple document level index. They resemble KadoP~\cite{DBLP:conf/icde/AbiteboulMPPS08} which, however, indexed at node granularity. Thus,  for each element name $a$, a KadoP peer stored the identifiers of all elements labeled $a$ in all documents in the system. The ViP2P document-granularity views are also related to DHT-based XML document indexing. We could in fact improve ViP2P's fallback option by adopting one of the approaches discussed in Section~\ref{sec:state}, enabling one to efficiently locate in the peer network, the documents matching a given query. We do not pursue this further, as this work focuses on node-granularity views that allow computing query results without contacting publishers at query time.


==> views_queries_old.tex <==
%--------------------------------------------------
\Subsection{Views and queries}
\label{sec:views-queries}

Both views and queries are formulated in an expressive subset of XQuery, comprising FLWR expressions with value joins, XPath navigation and multiple returning nodes and subtrees. Internally (and for ease of explanation in this paper), we represent queries and views using by a dialect of joined tree patterns. A straightforward translation exists between the two representations, examples of which can be found in~\cite{rewritingICDE2011}.

Formally, a tree pattern is a tree in which each node is labeled either with an XML element or attribute name, or with some keyword. The latter allows expressing simple keyword searches such as ``find all \kwd{//article} elements whose \kwd{abstract} child elements contain the keyword XML''. Each  node may also be annotated with zero or more among the labels $ID$, $val$ and $cont$, denoting, respectively, whether the node identifier (or ID, in short), the string value of the element (obtained by concatenating all its text descendants) or the full XML subtree rooted at this node is needed. We support all these different levels of information corresponding to XML elements for the following reasons. The $cont$ is the natural granularity of XML query results (full XML subtrees are returned by the evaluation of an XPath query). The $val$ue of a node is used in the XQuery specification to determine whether two nodes are equal (e.g., whether the name of an employee is the same as the name of a car owner). Finally, storing node IDs allows combining data from several views, to compute query results out of partial results stored in the respective views. ViP2P implements several flavors of XML IDs, most notably the simple (start, end, depth) scheme intensively used in~\cite{DBLP:conf/icde/Al-KhalifaJPWKS02} and many follow-up works, as well as the rich ID scheme of~\cite{IDs} (also used in~\cite{DBLP:conf/icde/TangYOCW08}) and more resilient to updates. {\em In this paper, we adopt (start, end, depth) node identifiers} since they are the most widely used by now. Thus, to each node in an XML document we associate: the positional number of its start tag ({\em start}), the positional number of its end tag ({\em end}) and the depth at which the node lies in its XML document (thus, the root has depth 0, the root children have depth 1 etc.). Such IDs allow identifying if node $n_1$ is an ancestor of node $n_2$ by testing whether $n_1$.{\em start}$<$$n_2$.{\em start} and $n_1$.{\em end}$<$$n_2$.{\em end}. If this is the case, moreover, $n_1$ is the parent of $n_2$ iff $n_1$.{\em depth}+1=$n_2$.{\em depth}.

A pattern node may also be annotated with a value predicate of the form $[$=$c]$ where $c$ is some constant, imposing that the $val$ue of the respective element be equal to $c$. The pattern edges are either simple for parent-child relationships, double for ancestor-descendant relationships, or dashed for value joins. 

A joined tree pattern is a set of tree patterns, connected by value join edges. Each edge requires that the text value of one node in one pattern, be the same as the text value of a node in another patterns. We require that a joined pattern view be connected, i.e., we do not support views corresponding to a cartesian product of tree patterns.
Figure~\ref{fig:viewsAndQueries} shows some examples of views and queries.
